Generalized Sum Pooling for Metric Learning

A common architectural choice for deep metric learning is a convolutional neural network followed by global average pooling (GAP). Albeit simple, GAP is a highly effective way to aggregate information. One possible explanation for the effectiveness of GAP is considering each feature vector as representing a different semantic entity and GAP as a convex combination of them. Following this perspective, we generalize GAP and propose a learnable generalized sum pooling method (GSP). GSP improves GAP with two distinct abilities: i) the ability to choose a subset of semantic entities, effectively learning to ignore nuisance information, and ii) learning the weights corresponding to the importance of each entity. Formally, we propose an entropy-smoothed optimal transport problem and show that it is a strict generalization of GAP, i.e., a specific realization of the problem gives back GAP. We show that this optimization problem enjoys analytical gradients enabling us to use it as a direct learnable replacement for GAP. We further propose a zero-shot loss to ease the learning of GSP. We show the effectiveness of our method with extensive evaluations on 4 popular metric learning benchmarks. Code is available at: GSP-DML Framework

==> paper/figures/fig_ablation_mu.tex <==
% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------
\begin{wrapfigure}[13]{r}[-5pt]{0.475\linewidth}
\vspace{0mm}
\centering
  \centerline{\includegraphics[width=1.0\linewidth,keepaspectratio]{paper/figures/mu_effect.jpg}}
\caption{Effect of $\mu$ in CUB dataset with C2 loss. Shaded regions represent $\mp$\textit{std}.} %.
\label{fig:mu_effect}
\end{wrapfigure}%

==> paper/figures/fig_computation.tex <==
\begin{wrapfigure}[16]{r}[-5pt]{0.495\linewidth}
\vspace{0mm}
\centering
  \centerline{\includegraphics[width=1.0\linewidth,keepaspectratio]{paper/figures/computation_32.png}}
\caption{Efficiency of closed-form gradient. Shaded regions represent $\mp$\textit{std}.} %.
\label{fig:closedform_autodiff}
\end{wrapfigure}%




==> paper/figures/table_conb_bni.tex <==
% \usepackage{caption}
% \usepackage{booktabs}


\begin{table*}[]
	\centering
	\caption{Comparison with state-of-the-art methods on Stanford Online Products \cite{oh2016deep}, CARS196 \cite{krause2014submodular} and CUB-200-2011 \cite{wah2011caltech} datasets. Red: the overall best. Blue: the overall second best. Bold: the loss term specific best. }
	\label{tab:all_result_2}
	\resizebox{\textwidth}{!}{
	\begin{tabular}{lcccc|cccc|cccc} 
		\toprule
		& \multicolumn{4}{c|}{Stanford Online Products}                 & \multicolumn{4}{c|}{CARS196}                                                                           & \multicolumn{4}{c}{CUB-200-2011}                                                                       \\ 
		\cmidrule{2-13}
		Method                & R@1           & R@10          & R@100         & R@1000        & \multicolumn{1}{l}{R@1} & \multicolumn{1}{l}{R@2} & \multicolumn{1}{l}{R@4} & \multicolumn{1}{l|}{R@8} & \multicolumn{1}{l}{R@1} & \multicolumn{1}{l}{R@2} & \multicolumn{1}{l}{R@4} & \multicolumn{1}{l}{R@8}  \\ 
		\midrule
		Proxy-NCA  \cite{movshovitz2017no}           & 73.7          & -             & -             & -             & 73.2                    & 82.4                    & 86.4                    & 88.7                     & 49.2                    & 61.9                    & 67.9                    & 72.4                     \\
		Clustering \cite{song2017deep}           & 67.0          & 83.7          & 93.2          & -             & 58.1                    & 70.6                    & 80.3                    & 87.8                     & 48.2                    & 61.4                    & 71.8                    & 59.2                     \\
		HDC  \cite{yuan2017hard}                 & 69.5          & 84.4          & 92.8          & 97.7          & 73.7                    & 83.2                    & 89.5                    & 93.8                     & 53.6                    & 65.7                    & 77.0                    & 85.6                     \\
		HTL  \cite{ge2018deep}                 & 74.8          & 88.3          & 94.8          & 98.4          & 81.4                    & 88.0                    & 92.7                    & 95.7                     & 57.1                    & 68.8                    & 78.7                    & 86.5                     \\
		MS   \cite{Wang_2019_CVPR_MS}                 & 78.2          & 90.5          & 96.0          & 98.7          & 84.1                    & 90.4                    & 94.0                    & 96.5                     & 65.7                    & \color[HTML]{FE0000}77.0                    & \color[HTML]{FE0000}86.3                    & \color[HTML]{FE0000}91.2                     \\
		TML    \cite{Yu_2019_ICCV}               & 78.0          & 91.2          & \color[HTML]{3166FF}96.7          & 99.0          & \color[HTML]{FE0000}86.3                    & \color[HTML]{3166FF}92.3                    & \color[HTML]{FE0000}95.4                    & 97.3                     & 62.5                    & 73.9                    & 83.0                    & 89.4                     \\ 
		\hline
		Margin   \cite{wu2017sampling}            & 72.7          & 86.2          & 93.8          & 98.0          & 79.6                    & 86.5                    & 91.9                    & 95.1                     & 63.6                    & 74.4                    & 83.1                    & 90.0                     \\
		M-PROFS               & 76.5          & 89.0          & 95.2          & \textbf{98.5} & 81.1                    & \textbf{88.1}           & 92.7                    & \textbf{95.8}            & \textbf{64.9}           & \textbf{75.8}           & \textbf{84.2}           & \textbf{90.4}            \\
		M-PROFS-HNCM          & \textbf{78.4} & \textbf{89.7} & \textbf{95.3} & \textbf{98.5} & \textbf{81.3}           & 88.0                    & \textbf{93.0}           & \textbf{95.8}            & 64.1                    & 75.0                    & \textbf{84.2}           & 90.3                     \\ 
		\midrule
		SoftTriple \cite{Qian_2019_ICCV}            & 78.3          & 90.3          & 95.9          & -             & 84.5                    & 90.7                    & 94.5                    & 96.9                     & 65.4                    & 76.4                    & 84.5                    & 90.4                     \\
		SoftTriple-PROFS      & \color[HTML]{3166FF}80.6          & \color[HTML]{3166FF}92.2          & 96.4          & \color[HTML]{3166FF}99.1          & \color[HTML]{3166FF}86.1                    & 91.9                    & 94.7                    & \color[HTML]{3166FF}97.4                     &\color[HTML]{FE0000} \textbf{66.3}           & \color[HTML]{3166FF}\textbf{76.8}           & \color[HTML]{3166FF}\textbf{85.0}           & \color[HTML]{3166FF}\textbf{90.7}            \\
		SoftTriple-PROFS-HNCM & \color[HTML]{FE0000}\textbf{81.7} &\color[HTML]{FE0000} \textbf{93.0} & \color[HTML]{FE0000}\textbf{96.8} &\color[HTML]{FE0000} \textbf{99.2} & \color[HTML]{FE0000}\textbf{86.3}           & \color[HTML]{FE0000}\textbf{92.5}           & \color[HTML]{3166FF}\textbf{95.0}           & \color[HTML]{FE0000}\textbf{97.5}            & \color[HTML]{3166FF}65.9                    & 76.2                    & 84.5                    & 90.6                     \\
		\bottomrule
	\end{tabular}}
\end{table*}
